Snippet-based Conversational Recommender System

Conversational Recommender Systems (CRS) engage users in interactive dialogues to gather preferences and provide personalized recommendations. While existing studies have advanced conversational strategies, they often rely on predefined attributes or expensive, domain-specific annotated datasets, which limits their flexibility in handling diverse user preferences and adaptability across domains. We propose SnipRec, a novel resource-efficient approach that leverages user-generated content, such as customer reviews, to capture a broader range of user expressions. By employing large language models to map reviews and user responses into concise snippets, SnipRec represents user preferences and retrieves relevant items without the need for intensive manual data collection or fine-tuning. Experiments across the restaurant, book, and clothing domains show that snippet-based representations outperform document- and sentence-based representations, achieving Hits@10 of 0.25-0.55 with 3,000 to 10,000 candidate items while successfully handling free-form user responses.

==> discussion.tex <==

% \section{Future Directions}\label{sec:discussion}

% \nikita{We explored alternative design choices, but they did not yield promising results, indicating a need for further research. For example, while snippets can be canonicalized to improve retrieval, our attempts to cluster them faced challenges due to uneven topic distribution (e.g., service vs. specific food items) and compositionality (e.g., ``fresh fruit'' linked to both freshness and fruit).  This further complicates determining the optimal $k$ for retrieval--too few snippets risk missing the target, while too many increase the overhead on the NLI model. While we assume the seeker has a specific target item in mind, multiple items may fulfill the preferences expressed in the snippets. An alternative setting could involve users interested in multiple target items. Future research should focus on optimizing snippet representation, determining the ideal $k$ for retrieval, and modeling user preferences.}

%Additionally, we simplify our approach by not factoring in other signals, like item and review popularity, during re-ranking.}

% \nikita{The quality of clarification questions generation varies across LLMs, with GPT-4o-mini significantly outperforming llama-3. This can be attributed to differences in their implicit knowledge of the restaurant domain. To explore this, we tested an alternative strategy that clusters the top 100 ranked items and extracts the top 10 topics from their associated snippets to generate questions. This approach outperformed llama-3. We include more details in the Appendix \todo{ref}.}

% \nikita{Although we assume the seeker has a specific target item in mind, multiple items may satisfy the preferences expressed in the snippets of the target item. A potential alternative setting could involve the user being interested in multiple target items, which we leave for future work.




% \subsection{Data Preprocessing}

% \paragraph{Snippets extraction}

% The acquisition of snippets is conducted by prompting gpt-4o-mini, which is economic and performs well for most of the time, but it still struggles with rhetoric languages, like ``this place could be for Bro's and Ho's in Philly to show their mating rituals'' \haibo{need another example}, which contains slangs and metaphors. However, LLaMa 3 is bad at extracting snippets and cannot follow the examples. \todo{example} as shown in Appendix. 

% For llama 3's defect, it could be possible that prompting engineering is different for llama-series at least totally different from GPT series. 

% \paragraph{Canonicalization}

% We tried canonicalization to reduce the number of snippets and combine those with similar meaning but this a quite challenging problem.

% Clustering is proved to work for simple cases like named entities or user query type \cite{viswanathan2023large, wan2024tnt}, but it is challenging to work with snippets in restaurant domain.

% The result we observed is that, some major topics such as service and atmosphere will occupy more than one clusters, while some long-tail topics such as kids' places or a comment to a specific food such as fried chicken are usually mixed with other snippets.

% Besides the uneven distribution, a snippet is still compositional in terms of its facets, such as ``fresh vegetable'', it can be grouped with both ``freshness'' and ``vegetable''. This adds to the complexity of this problem.

% We propose that some data rebalance methods or merge-based method can be used for this end, and a better definition of the problem is needed in future work.

% \paragraph{Vector Retrieval}

% In vector retrieval, the setting of the value for $k$ should be a moderate one—not too small and not too large. If $k$ is set too small, it may result in insufficient retrieval, as many snippets have not undergone canonicalization and are semantically similar, causing the target item to be missed. On the other hand, if **k** is set too large, items with significant semantic differences may also be retrieved. Although NLI filtering helps, the retrieved items may still not have the closest meaning, which can cause the target item to be overshadowed by irrelevant items.


% \subsection{Algorithms}

% \paragraph{Reranking algorithm}

% Weights are evenly distributed among all intents, but some intents are more unique than others so that they should be prioritized. It is possible that some domain-specific trained ranking or fine-tuned LLM are introduced to assign weights to different intents.

% \haibo{Popularity of items are not yet considered. In our algorithm the value is 1:0 outperforms 5:2, but 5:2 is more popular item and may need to be considered some bonus. Did we solve popularity problem?}

% \paragraph{Clarification question strategy}

% gpt-4o-mini works generall well in generating clarification questions given certain item profiles and conversation history, but llama-3 fall short on this. This indicates that the implicit knowledge in restaurant domain has some difference between these two models.

% We also tried another strategy in generating clarification questions aside from using LLM, which is based on on-the-fly clustering of top 100 items of current ranking and find the top 10 topics of 1000 sampled non-retrieved snippets associated with these top-ranking items. This method works better than llama-3, meaning that there are more internal connections underneath the topic distribution of certain kinds of user preferences, which is better encoded in gpt-4o-mini but less in llama-3. Details can be seen in Appendix.

% \haibo{Actually data-ask is better than llama-3...}

% \paragraph{Enhancement}

% Inspired by previous work \cite{xu2024personalized, lyu2023llm}, we implemented 3 kinds of augmentation part in the system. We observe that paraphrase does help, and support may help, but occurence not helps. This indicates that it's better to have correct augmentation than incorrect ones. 

% \subsection{Evaluation Methods}

% \paragraph{Task Validity}

% We observe that most of the time, while the user writes some best reviews, it is not essentially the best restaurant for the user, based on the limited information expressed in user review.

% The selection of one-best item may not be the most suitable for evaluating our system. The one selected item may lack popularity and not the best choice of the user, and their rivals can be ranked ahead of the answer and are essentially better than the item, but there is no metric for this.

% Possible better tasks may include ranking multiple items by the same user. This requires a even bigger dataset.

% -- nikita: we can skip this since we cover this assumption in the earlier sections.
% \paragraph{User Behavior Simulation}

% User answers can be more complex, such as regretting previous utterance \cite{\todo{cite}}, fuzzy responses \cite{shen2024multi} and critique \cite{critique}. This requires the interface-level design to adjust user's preferences and infer potential preferences and dislikes from critiques. In our case we only consider the user expressing preferences and dislikes to simplify our task. 

% Given the response to be free-form rather than templated, the critical point of a simulation of user is that: to what extent can a human react to a fuzzy question? A good question needs to be in the middle of being too general and too detailed, at a place that exactly provokes the maximum thought from the user. 

% On the other hand, human user will provide bad quality answer to ill-formed questions. Thus, one limitation of our user simulator is that unlike human users who will not provide enough information, user simulators will be very polite and informative.


% \subsection{Connection to previous methods}

% Embedding based methods can be viewed as some uninterpretable reasoning process or domain-specific connection. This analysis methods can be enhanced by having more known pairs that the LLM can be prompted to do such reasoning. For example, if the user is determined by the system to be of some personality (either implicitly or explicitly), the system can infer the user may like some kinds of cuisine; this can be ``enhanced query''. Our current setting shows that simply enhancement with commonsense knowledge isn't that making sense because we don't know the user much.

% Attribute-based methods can be seen as operating on a limited space. We also adopted the idea of facet-based but not necessarily a pre-defined facets, but more dynamically generated.
